A Chekanov-Eliashberg algebra for Legendrian graphs

We define a differential graded algebra for Legendrian graphs and tangles in the standard contact Euclidean three space. This invariant is defined combinatorially by using ideas from Legendrian contact homology. The construction is distinguished from other versions of Legendrian contact algebra by the vertices of Legendrian graphs. A set of countably many generators and a generalized notion of equivalence are introduced for invariance. We show a van Kampen type theorem for the differential graded algebras under the tangle replacement. Our construction recovers many known algebraic constructions of Legendrian links via suitable operations at the vertices.

==> RM_Base_a_input.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'RM_Base_a.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{76.47929057bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.67191113)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{RM_Base_a.pdf}}%
    \put(0.72128314,0.58433213){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_1$}}}%
    \put(-0.00434145,0.46421881){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_6$}}}%
    \put(0.80905268,0.34154722){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_2$}}}%
    \put(0.78406929,0.19777489){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_3$}}}%
    \put(0.64064277,0.01233483){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_4$}}}%
    \put(0.00375472,0.21045194){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_5$}}}%
    \put(0.41002718,0.22270888){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_0$}}}%
    \put(0.42404205,0.42191007){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfw$}}}%
    \put(0.44586242,0.09922902){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfv^j$}}}%
  \end{picture}%
\endgroup%


==> RM_Base_b_input.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'RM_Base_b.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{77.58085307bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.66237073)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{RM_Base_b.pdf}}%
    \put(0.71104172,0.57603526){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_1'$}}}%
    \put(-0.00427981,0.45762741){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_6'$}}}%
    \put(0.79756502,0.33669763){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_2'$}}}%
    \put(0.77293637,0.19496671){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_3'$}}}%
    \put(0.63154635,0.01215969){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_4'$}}}%
    \put(0.00370141,0.20746375){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_5'$}}}%
    \put(0.30235296,0.22299946){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_0'$}}}%
    \put(0.41802112,0.41591941){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfw'$}}}%
    \put(0.18728006,0.30082275){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfv'^j$}}}%
  \end{picture}%
\endgroup%


==> canonicalpath_vertex2_0-5_input.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'canonicalpath_vertex2_0-5.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{65.76558655bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.53631109)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{canonicalpath_vertex2_0-5.pdf}}%
    \put(0.5116696,0.34089507){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfv'$}}}%
    \put(0.88411191,0.47951022){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfh_{\sfv'\!,i}$}}}%
    \put(0.69256486,0.08080419){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\theta$}}}%
    \put(-0.00292199,0.30788468){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfh_{\sfv'\!,i+1}$}}}%
  \end{picture}%
\endgroup%


==> canonicalpath_vertex2_0_input.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'canonicalpath_vertex2_0.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{65.76558655bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.5381223)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{canonicalpath_vertex2_0.pdf}}%
    \put(0.5116696,0.34270628){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfv'$}}}%
    \put(0.88411191,0.48132143){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfh_{\sfv'\!,i}$}}}%
    \put(0.69256486,0.0826154){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\theta$}}}%
    \put(-0.00292199,0.30969589){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfh_{\sfv'\!,i+1}$}}}%
  \end{picture}%
\endgroup%


==> canonicalpath_vertex2_1_input.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'canonicalpath_vertex2_1.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{65.76558655bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.53631109)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{canonicalpath_vertex2_1.pdf}}%
    \put(0.5116696,0.34089507){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfv'$}}}%
    \put(0.88411191,0.47951022){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfh_{\sfv'\!,i}$}}}%
    \put(0.69256486,0.08080419){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\theta$}}}%
    \put(-0.00292199,0.30788468){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfh_{\sfv'\!,i+1}$}}}%
  \end{picture}%
\endgroup%


==> canonicalpath_vertex_0-5_input.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'canonicalpath_vertex_0-5.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{67.69653121bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.75604374)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{canonicalpath_vertex_0-5.pdf}}%
    \put(0.20349236,0.43439707){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfv$}}}%
    \put(0.65717401,0.6152233){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfh_{\sfv,i}$}}}%
    \put(0.49241861,0.34844868){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\theta$}}}%
    \put(0.66258577,0.18732924){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfh_{\sfv,i+1}$}}}%
  \end{picture}%
\endgroup

==> canonicalpath_vertex_0_input.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'canonicalpath_vertex_0.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{67.69653121bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.75604374)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{canonicalpath_vertex_0.pdf}}%
    \put(0.20349236,0.43439707){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfv$}}}%
    \put(0.65717401,0.6152233){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfh_{\sfv,i}$}}}%
    \put(0.49241861,0.34844868){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\theta$}}}%
    \put(0.66258577,0.18732924){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfh_{\sfv,i+1}$}}}%
  \end{picture}%
\endgroup%

==> canonicalpath_vertex_1_input.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'canonicalpath_vertex_1.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{67.69653121bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.75604374)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{canonicalpath_vertex_1.pdf}}%
    \put(0.20349236,0.43439707){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfv$}}}%
    \put(0.65717401,0.6152233){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfh_{\sfv,i}$}}}%
    \put(0.49241861,0.34844868){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\theta$}}}%
    \put(0.66258577,0.18732924){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfh_{\sfv,i+1}$}}}%
  \end{picture}%
\endgroup%


==> edge_contraction_1_input.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'edge_contraction_1.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{78.86717356bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.64649862)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{edge_contraction_1.pdf}}%
    \put(0.71674002,0.57217011){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_1$}}}%
    \put(0.78507124,0.43527744){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_2$}}}%
    \put(0.80188209,0.3236058){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_3$}}}%
    \put(0.77906734,0.19992574){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_4$}}}%
    \put(0.64337967,0.01020307){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_5$}}}%
    \put(0.01417307,0.17831231){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_6$}}}%
    \put(-0.00383853,0.32120486){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_7$}}}%
    \put(0.03218474,0.45809258){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_8$}}}%
  \end{picture}%
\endgroup%


==> edge_contraction_2_input.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'edge_contraction_2.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{81.08368967bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.62628893)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{edge_contraction_2.pdf}}%
    \put(0.69714711,0.55652918){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_1'$}}}%
    \put(0.76361041,0.43741819){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_2'$}}}%
    \put(0.79400142,0.30650117){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_3'$}}}%
    \put(0.75777063,0.17216249){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_4'$}}}%
    \put(0.62579214,0.00992416){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_5'$}}}%
    \put(0.02369604,0.16683067){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_6'$}}}%
    \put(-0.0037336,0.31242436){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_7'$}}}%
    \put(0.03130493,0.45382798){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_8'$}}}%
    \put(0.42600463,0.37105338){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\fp_0'$}}}%
  \end{picture}%
\endgroup%


==> ribbon_example_input.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'ribbon_example.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{111.39743257bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,1.01013403)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{ribbon_example.pdf}}%
    \put(0.27792325,0.66279013){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\gamma_1$}}}%
    \put(0.49069307,0.4710147){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\gamma_2$}}}%
    \put(0.27341253,0.29308039){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\gamma_3$}}}%
    \put(0.06421945,0.48544147){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\gamma_4$}}}%
    \put(-0.00815282,0.64831432){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Lambda_1$}}}%
    \put(-0.00815282,0.27624928){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Lambda_2$}}}%
    \put(0.49920049,0.84548462){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfa_1$}}}%
    \put(0.5031041,0.11276372){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfa_2$}}}%
    \put(0.28038935,0.92723827){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfv^1$}}}%
    \put(0.27335238,0.01898818){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfv^2$}}}%
    \put(0.30683902,0.57617834){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfw$}}}%
  \end{picture}%
\endgroup%


==> tangle_replacement_1_input.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'tangle_replacement_1.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{48.39999949bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,1.00745194)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{tangle_replacement_1.pdf}}%
    \put(0.43692698,0.60868663){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfw$}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{tangle_replacement_1.pdf}}%
  \end{picture}%
\endgroup%


==> tangle_replacement_2_input.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'tangle_replacement_2.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{52.15461066bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.92800928)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{tangle_replacement_2.pdf}}%
    \put(0.50258317,0.54804806){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfw^1$}}}%
    \put(0.6315043,0.30564137){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfw^3$}}}%
    \put(0.29016996,0.54597434){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfw^4$}}}%
    \put(0.13760948,0.30654763){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\sfw^2$}}}%
  \end{picture}%
\endgroup%

